sPIN: High-performance streaming Processing in the Network

Optimizing communication performance is imperative for large-scale computing because communication overheads limit the strong scalability of parallel applications. Today's network cards contain rather powerful processors optimized for data movement. However, these devices are limited to fixed functions, such as remote direct memory access. We develop sPIN, a portable programming model to offload simple packet processing functions to the network card. To demonstrate the potential of the model, we design a cycle-accurate simulation environment by combining the network simulator LogGOPSim and the CPU simulator gem5. We implement offloaded message matching, datatype processing, and collective communications and demonstrate transparent full-application speedups. Furthermore, we show how sPIN can be used to accelerate redundant in-memory filesystems and several other use cases. Our work investigates a portable packet-processing network acceleration model similar to compute acceleration with CUDA or OpenCL. We show how such network acceleration enables an eco-system that can significantly speed up applications and system services.

==> Makefile <==
DOCUMENT=spin_arxiv


FILES=*.tex 

all: $(DOCUMENT).pdf 


$(DOCUMENT).pdf: $(FILES)
	if [ -f plt/Makefile ]; then make -C plt; fi
	if [ -f img/Makefile ]; then make -C img; fi
	if [ -d ../img ]; then make -C ../img; fi
	rm -f pdflatex.out
	make -C ../paper_src/rplot
	cp ../paper_src/rplot/*.pdf rplot/
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	if grep -q citation $(DOCUMENT).aux; then bibtex $(DOCUMENT); fi;
# don't use pdflatex due to transparency issues  
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out
	pdflatex $(DOCUMENT).tex 2>&1 | tee pdflatex.out

	mv $(DOCUMENT).pdf $(DOCUMENT).tmp.pdf
	gs -dCompatibilityLevel=1.4 -dPDFSETTINGS=/prepress -dCompressFonts=false -dSubsetFonts=true -dNOPAUSE -dBATCH -sDEVICE=pdfwrite -sOutputFile=$(DOCUMENT).pdf -c ".setpdfwrite <</NeverEmbed [ ]>> setdistillerparams" -f $(DOCUMENT).tmp.pdf
	rm $(DOCUMENT).tmp.pdf

	#dvips $(DOCUMENT).dvi -o $(DOCUMENT).ps
# use ps2pdf to avoid lossy image compression in pdf which looks ugly on the
# beamer
	#ps2pdf14 -dPDFSETTINGS=/printer -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode $(DOCUMENT).ps

copyin: ~/projekte/latex/macros/*
	cp ~/projekte/latex/macros/bibliography.bib .
	cp ~/projekte/latex/macros/htor.sty .
	cp ~/projekte/latex/macros/htor_paper.cls .

show: $(DOCUMENT).pdf
	evince $(DOCUMENT).pdf

spell:
	for i in $$(ls -1 *.tex); do \
		echo "checking $$i ... "; \
		aspell -t --lang=en_US --home-dir="$$(pwd)" -p aspell.en_US.dic -c $$i; \
done; \

force:
	touch $(DOCUMENT).tex
	make $(DOCUMENT).pdf

clean:
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	rm -f *.aux *.out $(DOCUMENT).bbl
	rm -f $(DOCUMENT).blg $(DOCUMENT).dvi $(DOCUMENT).vrb
	rm -f  $(DOCUMENT).toc $(DOCUMENT).lo[a,f,g,h,l,t]
	rm -f $(DOCUMENT).nav $(DOCUMENT).snm $(DOCUMENT).ps $(DOCUMENT).pdf
	rm -f aspell*dic
	if [ -f plt/Makefile ]; then make -C plt clean; fi
	if [ -d img ]; then make -C img clean; fi
	if [ -d slides ]; then make -C img clean; fi
	if [ -d ../img ]; then make -C ../img clean; fi
	cat *.tex *.c | md5sum

pack: $(DOCUMENT).tgz

$(DOCUMENT).tgz: *.tex
	mkdir $(DOCUMENT) 
	cp *.tex $(DOCUMENT)
	cp *.sty $(DOCUMENT)
	cp *.cls $(DOCUMENT)
	cp *.bib $(DOCUMENT)
	cp *.bst $(DOCUMENT)
	if [ -d img ]; then cp -a img $(DOCUMENT); fi
	if [ -d kivio ]; then cp -a kivio $(DOCUMENT); fi
	if [ -d rplot ]; then cp -a rplot $(DOCUMENT); fi
	if [ -d src ]; then cp -a src $(DOCUMENT); fi
	if [ -d dia ]; then cp -a dia $(DOCUMENT); fi
	cp Makefile $(DOCUMENT)
	make -C $(DOCUMENT)
	cp $(DOCUMENT)/$(DOCUMENT).pdf $(DOCUMENT)/$(DOCUMENT)_orig.pdf
	make -C $(DOCUMENT) clean
	tar czf $(DOCUMENT).tgz $(DOCUMENT) --exclude=.svn 
	tar tzf $(DOCUMENT).tgz
	rm -fr $(DOCUMENT)
	@echo "voila: $(DOCUMENT).tgz"

commit: clean 
	svn commit

update: clean 
	svn update

%.o: %.c ptl_mockup.h
	    gcc -std=c99 -O3 -c $< -o $@


